A Generalized Framework of Sequence Generation with Application to Undirected Sequence Models

Undirected neural sequence models such as BERT (Devlin et al., 2019) have received renewed interest due to their success on discriminative natural language understanding tasks such as question-answering and natural language inference. The problem of generating sequences directly from these models has received relatively little attention, in part because generating from undirected models departs significantly from conventional monotonic generation in directed sequence models. We investigate this problem by proposing a generalized model of sequence generation that unifies decoding in directed and undirected models. The proposed framework models the process of generation rather than the resulting sequence, and under this framework, we derive various neural sequence models as special cases, such as autoregressive, semi-autoregressive, and refinement-based non-autoregressive models. This unification enables us to adapt decoding algorithms originally developed for directed sequence models to undirected sequence models. We demonstrate this by evaluating various handcrafted and learned decoding strategies on a BERT-like machine translation model (Lample & Conneau, 2019). The proposed approach achieves constant-time translation results on par with linear-time translation results from the same undirected sequence model, while both are competitive with the state-of-the-art on WMT'14 English-German translation.

==> tables/constant-time.tex <==
\begin{center}
\begin{tabular}[b]{llcc}
\toprule
& & \multicolumn{1}{c}{WMT'14 De$\rightarrow$En} & \multicolumn{1}{c}{WMT'14 En$\rightarrow$De} \\
   \midrule
   \midrule
%\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize Our Model}}
    & Most-to-least; $K$\;=\;$1$, $T$\;=\;$L$ & 26.03 & 20.72 \\
    & Easy-first; $K$\;=\;$1$, $T$\;=\;$L$ & 26.03 & 20.72 \\
    \midrule
    & Most-to-least; $K$\;=\;$T \rightarrow 1$, $T$\;=\;10 & 26.03 & 20.72 \\
	& Easy-first; $K$\;=\;$T \rightarrow 1$, $T$\;=\;10 & 19.05 & 15.07 \\ 
	\midrule
	& Easy-first $K$\;=\;2, $T$\;=\;$L$ / 2 & \elman{TODO} & \elman{TODO}\\
	& Easy-first $K$\;=\;3, $T$\;=\;$L$ / 3 & \elman{TODO} & \elman{TODO}\\
    \bottomrule
\end{tabular}
\vspace{-2mm}
\caption{\alert{Number are outdated, do we still need to flex with constant machine translation }Effect of various hyperparameters to allow faster decoding from the model. Add decodings were ran using }
\end{center}

==> tables/generation-order-example-0.tex <==
\centering
\footnotesize
\begin{tabular}{cc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\color{orange} Outside-In} \\
\midrule
(source) & Mit Bitcoin ist Bezahlen und Verkaufen ohne Bank möglich \\
1 &  \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ \textbf{.} \\ 
2 &  \_ \textbf{@coin} \_ \_ \_ \_ \_ \_ \_ \_ \_ . \\ 
3 &  \_ @coin \_ \_ \_ \_ \_ \_ \_ \_ \textbf{bank} . \\ 
4 & \textbf{Bit} @coin \_ \_ \_ \_ \_ \_ \_ \_ bank . \\ 
5 & Bit @coin \_ \_ \_ \_ \_ \_ \_ \textbf{a} bank . \\ 
6 & Bit @coin \_ \_ \_ \_ \_ \_ \textbf{without} a bank . \\ 
7 & Bit @coin \_ \_ \_ \textbf{pay} \_ \_ without a bank . \\ 
8 & Bit @coin \_ \_ \textbf{to} pay \_ \_ without a bank . \\ 
9 & Bit @coin \_ \_ to pay \textbf{and} \_ without a bank . \\ 
10 & Bit @coin \_ \_ to pay and \textbf{sell} without a bank . \\ 
11 & Bit @coin \_ \textbf{possible} to pay and sell without a bank . \\ 
12 & Bit @coin \textbf{is} possible to pay and sell without a bank . \\
(target) & With Bitcoin , pay and sell without banks \\

\bottomrule
\end{tabular}

\caption{Example sentences generated following an {\color{orange} outside-in} generation order, using the \textbf{easy-first} decoding algorithm on De$\rightarrow$En. The order color matches the cluster color in Figure~\ref{fig:gen-order}, bottom left.}

==> tables/generation-order-example-1.tex <==
\centering
\footnotesize
\begin{tabular}{cc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\color{orange} Left-to-Right} \\
\midrule
(source) & Allerdings bleibt in diesem wichtigen Themenbereich noch viel zu tun . \\
1 &  \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ \textbf{.} \\ 
2 &  \_ , \_ \_ \_ \_ \_ \_ \_ \_ \_ \_ . \\ 
3 &  \_ , there \_ \_ \_ \_ \_ \_ \_ \_ \_ . \\ 
4 &  \_ , there is \_ \_ \_ \_ \_ \_ \_ \_ . \\ 
5 &  \_ , there is still \_ \_ \_ \_ \_ \_ \_ . \\ 
6 &  \_ , there is still much \_ \_ \_ \_ \_ \_ . \\ 
7 &  \_ , there is still much \_ \_ in \_ \_ \_ . \\ 
8 &  \_ , there is still much \_ do in \_ \_ \_ . \\ 
9 &  \_ , there is still much \_ do in \_ \_ area . \\ 
10 &  \_ , there is still much to do in \_ \_ area . \\ 
11 &  \_ , there is still much to do in this \_ area . \\ 
12 &  \_ , there is still much to do in this important area . \\ 
13 & However , there is still much to do in this important area . \\
(target) & However , in this vital area , much remains to be done . \\

\bottomrule
\end{tabular}

\caption{Example sentences generated following an {\color{orange} outside-in} generation order, using the \textbf{easy-first} decoding algorithm on De$\rightarrow$En. The order color matches the cluster color in Figure~\ref{fig:gen-order}, bottom left.}

==> tables/generation-order-example.tex <==
\centering
\footnotesize
\begin{tabular}{ccc}
%\begin{tabular}{cccccccccccccccccccc}
\toprule
Iteration & {\color{orange} Left-to-Right-to-Left} & {\color{blue} Right-to-Left} \\
\midrule
(source) & \makecell{Mit Bitcoin ist Bezahlen und \\ Verkaufen ohne Bank möglich} & \makecell{Wer auch immer versucht hat , \\ sich dieser Familie entgegenzustellen , \\ musste mit dem Leben dafür zahlen} \\
1 & \_ \textbf{Bit} \_ \_ \_ \_ \_ \_ \_ & \_ \_ \_ \_ \_ \_ \_ \_ \textbf{.} \\
2 & \textbf{With} Bit \_ \_ \_ \_ \_ \_ \_ & \textbf{Who} \_ \_ \_ \_ \_ \_ \_ . \\
3 & With Bit \textbf{@coin} \_ \_ \_ \_ \_ \_ & Who \_ \_ \_ \_ \_ \textbf{family} \_ . \\
4 & With Bit @coin \_ \_ \_ \_ \textbf{without} \_ & Who\_ \_ \_ \_ \_ family \textbf{died} . \\
5 & With Bit @coin \_ \_ \_ \_ without \textbf{banks} & Who\_ \_ \_ \_ \textbf{this} family died . \\
6 & With Bit @coin \_ \_ \textbf{and} \_ without banks & Who \_ \_ \_ \textbf{defy} this family died . \\
7 & With Bit @coin \_ \textbf{pay} and \_ without banks & Who \_ \_ \textbf{to} defy this family died . \\
8 & With Bit @coin \_ pay and \textbf{sell} without banks & Who \_ \textbf{attempted} to defy this family died . \\
9 & Bit @coin \textbf{is} possible to pay and sell without a bank . & Anyone \textbf{who} ever tried to deal with this family has had to pay for it with life . \\
(target) & With Bit @coin , pay and sell without banks & Who \textbf{@ever} attempted to defy this family died . \\

%1 & $<\_ \underline{Bit} $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ & $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ \underline{.} \\
%2 & \underline{With} Bit $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ & \underline{Who} $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ . \\
%3 & With Bit \underline{\#coin} $<\_ $<\_ $<\_ $<\_ $<\_ $<\_ & Who $<\_ $<\_ $<\_ $<\_ $<\_ \underline{family} $<\_ . \\
%4 & With Bit \#coin $<\_ $<\_ $<\_ $<\_ \underline{without} $<\_ & Who$<\_ $<\_ $<\_ $<\_ $<\_ family \underline{died} . \\
%5 & With Bit \#coin $<\_ $<\_ $<\_ $<\_ without \underline{banks} & Who$<\_ $<\_ $<\_ $<\_ \underline{this} family died . \\
%6 & With Bit \#coin $<\_ $<\_ \underline{and} $<\_ without banks & Who $<\_ $<\_ $<\_ \underline{defy} this family died . \\
%7 & With Bit \#coin $<\_ \underline{pay} and $<\_ without banks & Who $<\_ $<\_ \underline{to} defy this family died . \\
%8 & With Bit \#coin $<\_ pay and \underline{sell} without banks & Who $<\_ \underline{attempted} to def \#y this family died . \\
%9 & With Bit \#coin \underline{,} pay and sell without banks & Whoever \underline{\#ever} attempted to def \#y this family died . \\

%1 & $<\_ & \underline{Bit} & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & \underline{.} \\
%2 & \underline{With} & Bit & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & \underline{Who} & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & . \\
%3 & With & Bit & \underline{\#coin} & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & Who & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & \underline{family} & $<\_ & . \\
%4 & With & Bit & \#coin & $<\_ & $<\_ & $<\_ & $<\_ & \underline{without} & $<\_ & Who & $<\_ & $<\_ & $<\_ & $<\_ & $<\_ & family & \underline{died} . \\
%5 & With & Bit & \#coin & $<\_ & $<\_ & $<\_ & $<\_ & without & \underline{banks} & Who & $<\_ & $<\_ & $<\_ & $<\_ & \underline{this} & family & died & . \\
%6 & With & Bit & \#coin & $<\_ & $<\_ & \underline{and} & $<\_ & without & banks & Who & $<\_ & $<\_ & $<\_ & \underline{defy} & this & family & died & . \\
%7 & With & Bit & \#coin & $<\_ & \underline{pay} & and & $<\_ & without & banks & Who & $<\_ & $<\_ & \underline{to} & defy & this & family & died & . \\
%8 & With & Bit & \#coin & $<\_ & pay & and & \underline{sell} & without & banks & Who & $<\_ & \underline{attempted} & to & defy & this & family & died & . \\
%9 & With & Bit & \#coin & \underline{,} & pay & and & sell & without & banks & Whoever & \underline{\#ever} & attempted & to & defy & this & family & died & . \\
\bottomrule
\end{tabular}

\caption{Example sentences generated following a {\color{orange} left-to-right-to-left} (left) and a {\color{blue} right-to-left} (right) order, using the easy-first decoding algorithm on De$\rightarrow$En. The order color matches the cluster color in Figure~\ref{fig:gen-order}, bottom left.}
